Neurotoxin: Durable Backdoors in Federated Learning

Due to their decentralized nature, federated learning (FL) systems have an inherent vulnerability during their training to adversarial backdoor attacks. In this type of attack, the goal of the attacker is to use poisoned updates to implant so-called backdoors into the learned model such that, at test time, the model's outputs can be fixed to a given target for certain inputs. (As a simple toy example, if a user types "people from New York" into a mobile keyboard app that uses a backdoored next word prediction model, then the model could autocomplete the sentence to "people from New York are rude"). Prior work has shown that backdoors can be inserted into FL models, but these backdoors are often not durable, i.e., they do not remain in the model after the attacker stops uploading poisoned updates. Thus, since training typically continues progressively in production FL systems, an inserted backdoor may not survive until deployment. Here, we propose Neurotoxin, a simple one-line modification to existing backdoor attacks that acts by attacking parameters that are changed less in magnitude during training. We conduct an exhaustive evaluation across ten natural language processing and computer vision tasks, and we find that we can double the durability of state of the art backdoors.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/results.tex <==
\subsection{Experimental Results}\label{sec:main-results}

In this subsection, we will display results for Task 1, and we will see that \algoname{} is significantly more durable than the baseline across multiple triggers.
We will also perform ablations to validate that this performance is robust across a range of algorithm and system hyperparameters and ensure that it does not degrade benign accuracy.
Lastly we will summarize the performance of \algoname{} across the remaining tasks.
Keeping in mind space constraints, because Task~1 is the common task across prior work and the most similar to real world FL deployments, we show full results on the remaining tasks in Appendix \ref{appendix:experiments}.
% \prateek{in which figure?}
% \prateek{where is all this summarized? consider rephrasing a bit}

\noindent \textbf{\algoname{} improves durability.}
% \noindent \textbf{Impact of mask ratio k on durability}\label{sec:main-results}
Fig. \ref{fig:ablation-lifespan-ratio} shows the results of varying the ratio of masked gradients $k$ starting from 0 $\%$ (the baseline).
We observe that \algoname{} increases durability over the baseline as long as $k$ is small.
We conduct this hyperparameter sweep at the relatively coarse granularity of $1 \%$ to avoid potentially overfitting; prior work on top-$k$ methods in gradient descent has shown further marginal improvements between $0 \%$ and $1 \%$~\cite{rothchild2020fetchsgd, panda2021sparsefed}.
Even with minimal hyperparameter tuning we see that there is a range of values of $k$ where \algoname{} outperforms the baseline.
As we reduce $k$, the lifespan improves until the difficulty of the constrained optimization outweighs the increased durability.
% \prateek{need to give some insight into the trends that we observe in figure 2 as the hyperparameter is varied. e.g., lifespan improves as k reduces until a threshold, at which point benign accuracy etc might suffer too?}
We expect that because there is a single hyperparameter to choose, and $k$ can be tuned in a single device simulation with a sample from the benign training distribution, the attacker will easily be able to tune the correct value of $k$ for their backdoor task.
% \prateek{would it be clear to the reader how the attacker would do the simulation? what knowledge about data distribution etc would the attacker need to have?}


%%%%% fig:ablation-lifespan-ratio %%%%% Reddit LSTM Lifespan vs Gradmaskratio
\begin{figure}[t] %[H]
\centering
\includegraphics[width=0.49\linewidth]{./figures/Reddit_LSTM/Lifespan_LSTM_Reddit_diff_trigger_diff_gradmask_ratio.pdf}
 \caption{%\footnotesize
 Impact of adjusting the mask ratio $k$ on the Lifespan for Task 1. AttackNum = 80, i.e., attacker participates in 80 rounds of FL. The 3 triggers here correspond to the first 3 rows of Tab.\ref{table:trigger-sentences}.
}
\label{fig:ablation-lifespan-ratio}
\end{figure}

% \noindent \textbf{\algoname{} improves durability
\noindent \textbf{\algoname{} makes hard attacks easier.}
Fig \ref{fig:task-1} compares the baseline and \algoname{} on Task 1 across all three triggers.
\algoname{} outperforms the baseline across all triggers, but the largest margin of improvement is on triggers 1 and 2 that represent ``base case'' attacks.
The words in triggers 1 and 2 are very common in the dataset, and the baseline attack updates coordinates frequently updated by benign devices.
We can consider triggers 1 and 2 to be ``hard'' attacks.
As a direct consequence, the baseline attack is erased almost immediately.
Trigger 3 includes the attack of ~\cite{wang2020attack}, where ``Roads in Athens'' can be considered an edge-case phrase.
The baseline attack lasts longer in this easier setting, but it is still outperformed significantly by \algoname{}.
The rest of our experiments follow this trend generally: the gap between \algoname{} and the baseline attack varies with the difficulty of the backdoor task.

%%%%% fig:task-1 %%%%% Reddit LSTM Lifespan vs Epoch
\begin{figure}
    \centering
    \includegraphics[width=0.32\linewidth]{./figures/Reddit_LSTM/Reddit_LSTM Sentence0_AttackNum40_acc.pdf}
    \includegraphics[width=0.32\linewidth]{./figures/Reddit_LSTM/Reddit_LSTM Sentence1_AttackNum40_acc.pdf}
    \includegraphics[width=0.32\linewidth]{./figures/Reddit_LSTM/Reddit_LSTM Sentence2_AttackNum40_acc.pdf}
    
    \caption{
    \textbf{Task 1 (Reddit, LSTM)} with triggers 1 (left), 2 (middle), 3 (right).
    AttackNum = 40.
    % \yaoqing{From Figure 2 to Figure 9, shall we put some bold text or text with brackets at the beginning to give a title to each set of figures? For example, Figure 2 can have a title like (Standard setting, LSTM on Reddit.) This way of summarizing the figure could help long captions in, say, Figure 7.}
    % Attack accuracy of neurotoxin on Reddit dataset with (Top) LSTM and (Bottom) GPT2 with (Left) first kinds of poision sentences, (Middle) second kinds of poision sentences, and (Right) third kinds of poision sentences. Start round of the attack of LSTM and GPT2 are 2000 and 0, respectively. Attack number of all of them is 40.
    }
    \label{fig:task-1}
\end{figure}

\noindent \textbf{\algoname{} empowers weak attackers and strong attackers alike.}
Fig. \ref{fig:task-1-lifespan-attacknum} compares \algoname{} and the baseline under various values of the AttackNum parameter (the number of consecutive epochs where the attacker is participating).
% \addressedmichael{AttackNum is usually not in quotes, why is it here, we need to be consistent.}
Because \algoname{} is performing constrained optimization, we expect that it will converge slower than the baseline.
Indeed, \algoname{} does not display as much improvement for a low number of attack epochs, because it takes more epochs to reach 100 $\%$ accuracy on the poisoned dataset.
However, even for the minimum number of epochs needed for the baseline attack to reach 100 $\%$ accuracy, that is AttackNum=40, \algoname{} is 
%still definitively 
significantly more durable.
The ``correct'' value of AttackNum may vary depending on the setting, so we perform the necessary ablations on a range of values of AttackNum.

%%%%% fig:task-1-lifespan-attacknum %%%%% Reddit LSTM Lifespan vs Attacknum
\begin{figure}
    \centering
    \includegraphics[width=0.32\linewidth]{./figures/Reddit_LSTM/Lifespan_LSTM_Reddit_trigger0_diff_attacknum.pdf}
    \includegraphics[width=0.32\linewidth]{./figures/Reddit_LSTM/Lifespan_LSTM_Reddit_trigger1_diff_attacknum.pdf}
    \includegraphics[width=0.32\linewidth]{./figures/Reddit_LSTM/Lifespan_LSTM_Reddit_trigger2_diff_attacknum.pdf}
    \caption{
    Lifespan on Reddit with different AttackNum. (Left) Trigger  1.  (Middle) Trigger  2.  (Right) Trigger  3. 
    }
    \label{fig:task-1-lifespan-attacknum}
\end{figure}

\noindent \textbf{\algoname{} makes single word trigger attacks possible.}
We consider the attacks we have evaluated so far to be impactful base case attacks.
The backdoor is triggered as soon as the user types ``\textit{race} people are'', where \textit{race} can be any skin color such as black, yellow, white, brown.
This trigger is a fairly common phrase.
% \michael{I'm not sure why race is in brackets or quotes.  Is the idea that we can substitute in different races later.  Clarify this par.}
In Fig. \ref{fig:task-1-triggerlen}, we consider an even stronger attack that interpolates between the base trigger sentence and a trigger sentence that consists only of ``\textit{race}''.
That is, if the backdoor corresponding to trigger length=1 is successfully implanted, then if the user types ``black'' the model will recommend `people', and if this suggestion is accepted, the model will recommend ``are'', until it finishes recommending the full backdoor, e.g. ``black people are psycho''.
% \prateek{we should have an ethical considerations discussion somewhere}
This backdoor is clearly more impactful and harder to implant than any backdoor seen in prior work: the backdoor is activated as soon as the user types a single common word; and the backdoor has a large impact because it recommends what can be regarded as hate speech.
% \prateek{good that we clearly ack our trigger phrase as hate speech. see if we can bring this up!}
We find that as we decrease the trigger length, increasing the difficulty and impact of the attack, the improvement of \algoname{} over the baseline increases.
In the case of trigger length=1, the baseline attack backdoor is erased in 32 rounds---less than half the number of epochs it took to insert the attack itself---while the \algoname{} backdoor lasts for nearly 4X longer, 122 rounds.

%%%%% Triggerlen belongs to Ablations?
%%%%% fig:task-1-triggerlen %%%%% Reddit LSTM Lifespan vs Triggerlen
\begin{figure}[t] 
    \centering
    \includegraphics[width=0.32\linewidth]{./figures/Reddit_LSTM/Reddit_LSTM_Sentence1_AttackNum80_predwords_len1_acc.pdf}
    \includegraphics[width=0.32\linewidth]{./figures/Reddit_LSTM/Reddit_LSTM_Sentence1_AttackNum80_predwords_len2_acc.pdf}
    \includegraphics[width=0.32\linewidth]{./figures/Reddit_LSTM/Reddit_LSTM_Sentence1_AttackNum80_predwords_len3_acc.pdf}
    \caption{
    Attack accuracy of baselline and \algoname{} on Reddit dataset with LSTM with different length trigger sentence. (Left) Trigger len = 3, means the trigger sentence is `\{race\} people are *', (Middle) trigger len = 2, means the trigger sentence is `\{race\} people * *', and (Right) trigger len = 1, means the trigger sentence is `\{race\} * * * ', where `race' is a random word selected from \{black brown yellow\} and `*' is the target word. 
    \michael{I changed some single quotes to double quotes, but then I stopped.  Would you go through and make things consistent everywhere.  I think everything should be double.  But I'm not sure why you are using single.}
    Start round and AttackNum of all experiments are 1800 and 80, respectively. The Lifespan of the baseline and neurotoxin are (Left) 78 and 123, (Middle) 54 and 93, (Right) 32 and 122.
    }
    \label{fig:task-1-triggerlen}
\end{figure}

\noindent \textbf{\algoname{} is robust to evaluated defenses.}
Fig. \ref{fig:task-1-defense-dp} shows experiments where the server implements differential privacy as a defense against the baseline attack and \algoname{}.
This evaluation mirrors~\cite{sun2019backdoor, wang2020attack}: the amount of noise added is much smaller than works that employ DP-SGD~\cite{abadi2016deep}; and it  does not degrade benign accuracy, but it may mitigate attacks.
% \prateek{what does a weak form of differential privacy mean?}
As a reminder, all our experiments include use of the norm clipping defense, where we tune the norm clipping parameter $L$ to the smallest value that does not degrade convergence in the benign setting.
These hyperparameter tuning experiments are available in Appendix~\ref{appendix:norm}.
\algoname{} is impacted more by noise addition than the baseline.
Baseline lifespan decreases from 17 to 13 (26 $\%$), and \algoname{} lifespan decreases from 70 to 41 (42 $\%$).
Noise is added to all coordinates uniformly and the baseline already experiences a `default noise level' because it is impacted by benign updates.
However, \algoname{} experiences a lower `default noise level' because it prefers to use coordinates that are not frequently updated by benign devices.
At a high level, the noise increase for the baseline when weak differential privacy is implemented server-side might look like $1 \rightarrow 1 + \epsilon$, while the same relation for \algoname{} could be $0 \rightarrow 0 + \epsilon$.
While both increases are identical in absolute terms, the relative increase is larger for \algoname{}, which can explain the impact on lifespan.
Even in the presence of this defense, \algoname{} still inserts backdoors that are more durable than those of the baseline.

%%%%%

\begin{figure}[ht]
\minipage{0.45\textwidth}
\includegraphics[width=\linewidth]{./figures/Reddit_LSTM/Baseline_Neurotoxin_with_DP.pdf}
 \caption{
 \footnotesize
 Task 1 (Reddit, LSTM) with trigger 2 (\{race\} people are *). AttackNum = 40, using differential privacy (DP) defense ($\sigma = 0.001$). The Lifespan of the baseline and \algoname{} are 13 and 41, respectively.
}
\label{fig:task-1-defense-dp}
\endminipage\hfill
\minipage{0.45\textwidth}
\includegraphics[width=\linewidth]{./figures/Reddit_LSTM/Baseline_Neurotoxin_half_participation.pdf}
 \caption{
 \footnotesize
 Task 1 (Reddit, LSTM) with trigger 2 (\{race\} people are *). AttackNum=80,  the attacker participate in 1 out of every 2 rounds. The Lifespan of the baseline and \algoname{} are 11 and 51, respectively.}
\label{fig:task-1-frequency-half}
\endminipage
\end{figure}

% \begin{figure}[ht]
% \minipage{0.23\textwidth}
% \includegraphics[width=\linewidth]{./figures/Reddit_LSTM/Reddit_LSTM Sentence0_AttackNum40_with_DP_acc.pdf}
%  \caption{
%  \footnotesize
%  Task 1 (Reddit, LSTM) with trigger 2 (\{race\} people are *). Attack number = 40, using differential privacy defense (noise power = 0.001). The Lifespan of the baseline and \algoname{} are 13 and 41, respectively.
% }
% \label{fig:task-1-defense-dp}
% \endminipage\hfill
% \minipage{0.23\textwidth}
% \includegraphics[width=\linewidth]{./figures/Reddit_LSTM/Reddit_LSTM_Sentence0_AttackNum80_interval2_acc.pdf}
%  \caption{
%  \footnotesize
%  Task 1 (Reddit, LSTM) with trigger 2 (\{race\} people are *). Attack number=80,  the attacker participate in 1 out of every 2 rounds. The Lifespan of the baseline and \algoname{} are 11 and 51, respectively.}
% \label{fig:task-1-frequency-half}
% \endminipage
% \end{figure}


%%%%%% With differential privacy defense 
% \begin{figure}
% \centering
% \includegraphics[width=0.65\linewidth]{./figures/Reddit_LSTM/Reddit_LSTM Sentence0_AttackNum40_with_DP_acc.pdf}
%  \caption{%\footnotesize
%  Task 1 (Reddit, LSTM) with trigger 2 ( black people are *). Attack number = 40, using differential privacy defense (noise power = 0.001). The Lifespan of the baseline and \algoname{} are 13 and 41, respectively.
% }
% \label{fig:task-1-defense-dp}
% \end{figure}

\noindent \textbf{\algoname{} is more durable under low frequency participation.}
The majority of our experiments take place in the fixed frequency setting where one attacker participates in each round where the attack is active.
Fig. \ref{fig:task-1-frequency-half} shows results where one attacker participates in 1 of every 2 rounds where the attack is active.
When compared to the full participation setting (Fig. \ref{fig:task-1-lifespan-attacknum}), we see that the baseline lifespan decreases from 17 to 11 (35 $\%$), and the \algoname{} lifespan decreases from 70 to 51 (27 $\%$).
This is in line with the rest of our results: the backdoor inserted by \algoname{} is more durable, so it is able to insert a better backdoor when the backdoor is being partially erased every other round.

\noindent \textbf{\algoname{} does not degrade benign accuracy.}
We include tables with all benign accuracy results across tasks in Appendix \ref{appendix:benign-acc}.
% \prateek{be specific about which appendix subsection etc}
Across all results, \algoname{} has the same minor impact on benign accuracy as the baseline.

%%%%%% With modified attack frequency
% \begin{figure}
% \centering
% \includegraphics[width=0.65\linewidth]{./figures/Reddit_LSTM/Reddit_LSTM_Sentence0_AttackNum80_interval2_acc.pdf}
%  \caption{%\footnotesize
%  Task 1 (Reddit, LSTM) with trigger 2 ( black people are *). Start attack round = 0,  attack end round is 80,  the attacker participate in 1 out of every 2 rounds. The Lifespan of the baseline and \algoname{} are 11 and 51, respectively.}
% \label{fig:task-1-frequency-half}
% \end{figure}

\noindent \textbf{\algoname{} performs well across all other tasks.}
We summarize performance on the remaining tasks.
Fig. \ref{fig:task-2} shows Task 2, where we replace the model architecture in Task 1 with the much larger GPT2.
We find that it is much easier to insert backdoors into GPT2 than any other task, and because of this \algoname{} does not significantly outperform the baseline.
To the best of our knowledge, this is the first time work has considered inserting backdoors during FL training into a model architecture on the scale of a modern Transformer.

Fig. \ref{fig:task-3-4} shows Tasks 3 and 4.
Because Tasks 3 and 4 are binary classification tasks, the (likely) lowest accuracy for the attack is 50 $\%$, and so we instead set the threshold accuracy to be 75 $\%$ in computing the lifespan.
The IMDB dataset is very easy to backdoor, so \algoname{} does not improve much over the baseline.
Sentiment140 is a harder task, and we do see a 2 $\times$ increase in durability.

Fig. \ref{fig:task-5-7} shows Tasks 5 and 7, the edge case attacks on CIFAR datasets.
The baseline attack here is the attack of ~\cite{wang2020attack}, modified to fit the few-shot setting.
\algoname{} again doubles the durability of the baseline for Task 5 (CIFAR10), but we are unable to evaluate the lifespan for Task 7 (CIFAR100).
That is, because the attacks are erased far too slowly, owing to the smaller amount of data each benign device has about the edge case backdoor.

Fig. \ref{fig:task-6-8} shows Tasks 6 and 8, the base case attacks on CIFAR datasets.
The baseline attack here is the attack of ~\cite{panda2021sparsefed}, modified to fit the few-shot setting.
\algoname{} more than doubles durability on CIFAR10.
There is a smaller gap on CIFAR100 because each benign device has less data pertaining to the base case backdoor and therefore the benign updates are less likely to erase the backdoor.

Fig. \ref{fig:task-9-10} shows Tasks 9 and 10, the edge case attacks on EMNIST datasets.
Task 9 uses the EMNIST-digit dataset that only contains the digits in the EMNIST dataset, and \algoname{} has a dramatic improvement over the baseline.
However, we are unable to evaluate the lifespan because \algoname{} is too durable and does not fall below the threshold accuracy for thousands of rounds.
Task 10 uses the EMNIST-byclass dataset that adds letters to EMNIST-digit.
Here, \algoname{} only has a marginal improvement over the baseline because the benign devices have less data about the backdoor.

\begin{figure}
    \centering
    \includegraphics[width=0.32\linewidth]{./figures/Reddit_GPT2/Reddit_GPT2_Sentence0_AttackNum40_acc.pdf}
    \includegraphics[width=0.32\linewidth]{./figures/Reddit_GPT2/Reddit_GPT2_Sentence1_AttackNum40_acc.pdf}
    \includegraphics[width=0.32\linewidth]{./figures/Reddit_GPT2/Reddit_GPT2_Sentence2_AttackNum40_acc.pdf}
    
    \caption{
    \textbf{Task 2} Attack accuracy of neurotoxin on Reddit dataset using the GPT2 architecture with (Left) trigger 1, (Middle) trigger 2, and (Right) trigger 3 (first 3 rows of~Tab. \ref{table:trigger-sentences}). Start round of the attack of LSTM and GPT2 are 2000 and 0, respectively. AttackNum=40.
    }
    \label{fig:task-2}
\end{figure}

\begin{figure*}
\centering
\begin{tabular}{cc|cc}
\includegraphics[width=0.22\linewidth]{./figures/Sentiment140_LSTM/Sentiment140_LSTM_Sentence2_AttackNum80_acc.pdf}&
\includegraphics[width=0.22\linewidth]{./figures/Sentiment140_LSTM/Sentiment140_LSTM_Sentence3_AttackNum80_acc.pdf}&

\includegraphics[width=0.22\linewidth]{./figures/IMDB_LSTM/IMDB_LSTM_Sentence0_AttackNum100_acc.pdf}&
\includegraphics[width=0.22\linewidth]{./figures/IMDB_LSTM/IMDB_LSTM_Sentence1_AttackNum100_acc.pdf}\\
\end{tabular}
 \caption{%\footnotesize
 \textbf{Tasks 3 and 4} Attack accuracy of \algoname{} on  (Left) Sentiment140 dataset and (Right) IMDB dataset. For Sentiment140, the first figure is the result of the trigger sentence `I am African American' and the second one is the result of the trigger sentence `I am Asian'.  For IMDB, the first and the second figures are the results of trigger 5 and 6 in Tab.\ref{table:trigger-sentences}. The round at which the attack starts is 150 for both datasets. AttackNum=80 and 100 for Sentiment140 and IMDB, respectively.
}
\label{fig:task-3-4}
\end{figure*}

\begin{figure}
\centering
\includegraphics[width=0.48\linewidth]{./figures/Cifar/cifar10_Resnet18_InDistributionCase0_AttackNum250_acc_train_longer.pdf}
\includegraphics[width=0.48\linewidth]{./figures/Cifar/cifar100_Resnet18_InDistributionCase0_AttackNum200_acc_train_longer.pdf}
 \caption{%\footnotesize
 \textbf{Tasks 5 and 7} Attack accuracy of \algoname{} on  (Left) CIFAR10 and (Right) CIFAR100. For each dataset, the trigger set is the same as \cite{wang2020attack}. The round at which the attack starts is 1800 for both datasets. AttackNum=200.
}
\label{fig:task-5-7}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.48\linewidth]{./figures/Cifar/cifar10_Resnet18_InDistributionCase1_AttackNum250_acc_train_longer.pdf}
\includegraphics[width=0.48\linewidth]{./figures/Cifar/cifar100_Resnet18_InDistributionCase1_AttackNum200_acc_train_longer.pdf}
 \caption{%\footnotesize
 \textbf{Tasks 6 and 8} Attack accuracy of \algoname{} on  (Left) CIFAR10 and (Right) CIFAR100. For CIFAR10 with base-case backdoor the lifespan of the baseline is 116, our \algoname{} is 279. For CIFAR100 with base-cased backdoor the lifespan of the baseline is 943, our \algoname{} is 1723. The round to start the attack is 1800 for both datasets. AttackNum of CIFAR10 and CIFAR100 is 250 and 200, respectively.
}
\label{fig:task-6-8}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.48\linewidth]{./figures/EMNIST/EMNIST_Digits_AttackNum200_acc.pdf}
\includegraphics[width=0.48\linewidth]{./figures/EMNIST/EMNIST_ByClass_AttackNum100_acc.pdf}
 \caption{%\footnotesize
 \textbf{Tasks 9 and 10} Attack accuracy of \algoname{} on (Left) EMNIST-digit and (Right) EMNIST-byclass. For each dataset, the trigger set is the same as \cite{wang2020attack}. AttackNum is 200 and 100, respectively. Attack start round is 1800 of both of them. 
}
\label{fig:task-9-10}
\end{figure}
